Spurious Lyapunov Exponents Computed Using the Eckmann-Ruelle Procedure

Lyapunov exponents can be difficult to determine from experimental data. In particular, when using embedding theory to build chaotic attractors in a reconstruction space, extra "spurious" Lyapunov exponents arise that are not Lyapunov exponents of the original system. By studying the local linearization matrices that are key to the Eckmann-Ruelle method for computing Lyapunov exponents, we determine explicit formulas for the spurious exponents in certain cases. Notably, when a two-dimensional system with Lyapunov exponents A and B is reconstructed in a five-dimensional space, we show that the reconstructed system has exponents A, B, 2A, A+B, 2B.

==> abstract.tex <==
\begin{abstract}

Lyapunov exponents, important invariants of a complicated dynamical
process, can be difficult to determine from experimental data.  In
particular, when using embedding theory to build chaotic attractors in a
reconstruction space, extra ``spurious'' Lyapunov exponents can arise that
are not Lyapunov exponents of the original system.  By studying the local
linearization matrices that are key to a popular method for computing
Lyapunov exponents, we determine explicit formulas for the spurious
exponents in certain cases.  Notably, when a two-dimensional system with
Lyapunov exponents $\alpha$ and $\beta$ is reconstructed in a
five-dimensional space, we show that the reconstructed system has
exponents $\alpha$, $\beta$, $2\alpha$, $2\beta$, and $\alpha+\beta$.

\end{abstract}

